CraftAssist: A Framework for Dialogue-enabled Interactive Agents

This paper describes an implementation of a bot assistant in Minecraft, and the tools and platform allowing players to interact with the bot and to record those interactions. The purpose of building such an assistant is to facilitate the study of agents that can complete tasks specified by dialogue, and eventually, to learn from dialogue interactions.

==> sec_intro_old.tex <==
{\color{blue}
% Yacine > tried to add some of the overall motivation without making any unsubstantiated claims and keeping the intro to the firs page
Machine learning systems that interact with and assist humans are expected to be able to complete a long tailed distribution of tasks. These can involve reasoning across multiple domains or interacting with an environment, and may be specified (often ambiguously) through natural language with few or no execution examples to learn from, or through multi-turn dialogue with humans.
Minecraft offers an unprecedented platform to train such a system (see \cite{} for a more detailed description of our motivations). This paper describes an in-game Bot assistant along with the tools and platform allowing players to interact with the bot and to record those interactions. In short, the purpose of building such an agent is to facilitate the study of the following:}
{\color{red}
% This paper describes an implementation of a Bot assistant in Minecraft, and the tools and platform allowing players to interact with the bot and to record those interactions.    For a detailed description of our motivations, see \cite{};  in short, the purpose of building such an agent is to facilitate the study of the following:
\newline
\noindent {\bf Synergies of machine learning (ML) components:} To explore and evaluate various approaches to building a complex agent. In particular, how ML and non-ML components of a system can work together, and how to exploit the synergies of these components.  Especially, how to exploit these components to make progress in:
%\newline
\newline
\noindent {\bf Grounded natural language understanding :}
How can we build a system to understand what a human wants; and to associate language to a task?   Here, specifying tasks is the challenge, not executing them.  
%advance the state of the art in grounded natural language understanding; and to provide a platform for ourselves and studying  grounded natural language understanding, together with our learning agents and training data, in order for the community to make fundamental advances.
\newline
\kavya{can we skip the self improvement bit here ? this sits well in the position paper but we don't have the implementation of this yet.}
\noindent {\bf Self improvement:}
To make progress in building agents with the ability to improve themselves during deployment and interaction with human players.  How to learn new tasks and concepts from dialogue or demonstrations?

\begin{figure}
    \centering \includegraphics[width=0.45\textwidth]{figures/bot.png}
    \caption{An in-game screenshot of a human player using in-game chat to communicate with the Bot.}
    \label{fig:screenshot_bot}
\end{figure}


The Bot appears and interacts like another player:  other players can observe the Bot moving around and modifying the world, and communicate with it via in-game chat. Figure \ref{fig:screenshot_bot} shows a screenshot of a typical in-game experience. The ultimate goal of the Bot is to be a useful and fun assistant in a wide variety of tasks specified and evaluated by human players.  Neither Minecraft nor the software framework described here provides an explicit objective or reward function. While longer term, we hope to build a Bot that interacts and collaborates with humans to actively learn new concepts and skills, the Bot described here should be taken as initial point from which we can bootstrap.

To encourage collaborative research, the code, data, and models are open-sourced. The design of the framework is purposefully modular to allow research on components of the Bot as well as the whole system. The released data includes the human actions used to build 2,586 houses, the labeling of the sub-parts of the houses (e.g., walls, roofs, etc.), human rewordings of templated commands, and the mapping of natural language commands to a Bot interpretable logical forms. To enable researchers to independently collect data, the infrastructure that allows for the recording of human and Bot interaction on a Minecraft server is also released. We hope these tools will help empower research on interactive Bots with rich task and communication abilities. 
}


Machine learning systems that interact with and assist humans are expected to be able to complete an open-ended and long tailed distribution of tasks. Many tasks may only be seen during training a few times, or even never, requiring sample efficiency and flexibility. Many of these tasks may also require reasoning across multiple domains, such as vision and language~\cite{VQApapers}, while simultaneously requiring the system to interact with an environment~\cite{EQApapers,interactiveenviron}. 

Challenges extend beyond just the diversity of the tasks. The task specification itself is often ambiguous, since it is typically communicated via natural language. Identifying and resolving ambiguities requires reasoning about the world and may involve engaging in multi-turn dialogue with humans. 

\begin{figure}
    \centering \includegraphics[width=0.45\textwidth]{figures/bot.png}
    \caption{An in-game screenshot of a human player using in-game chat to communicate with the bot. \lz{Let's use a screenshot with better exposure.}}
    \label{fig:screenshot_bot}
\end{figure}

We propose building an open-sourced interactive bot, and through it, the tools and platform for researching the ability to execute on interactive tasks specified through multi-turn dialogue. To support the bot, an environment is needed that allows for easy interaction with humans, has multi-modal inputs including language, and encourages a wide range of diverse tasks. We propose working in the sandbox construction game of Minecraft, which meets these requirements while offering a properly constrained scope that is amenable to research. Additional motivation on this research direction is provided in~\cite{positionpaper}. 

This paper describes an initial implementation of an assistant bot in Minecraft. The bot appears and interacts like another player. Human players can observe the bot moving around and modifying the world, and can communicate with it via in-game chat. Figure \ref{fig:screenshot_bot} shows a screenshot of a typical in-game experience. The ultimate goal of the bot is to be a useful and fun assistant in a wide variety of tasks specified and evaluated by human players. Neither Minecraft nor the software framework described here provides an explicit objective or reward function. Longer term, we hope to provide a bot that can interact and collaborate with humans to actively learn new concepts and skills through human interaction. 

To encourage collaborative research, the code, data, and models are open-sourced. The design of the framework is purposefully modular to allow research on sub-tasks, as well as, the complete bot. The released data includes the human actions used to build 2,586 houses, the labeling of the sub-parts of the houses (e.g., walls, roofs, etc.), human rewordings of templated commands, and the mapping of natural language commands to bot interpretable logical forms. To enable researchers to independently collect data, the infrastructure that allows for the recording of human and bot interaction on a Minecraft server is also released. We hope these tools will help empower research on interactive bots with rich task and communication abilities. 

